Agents and Devices: A Relative Definition of Agency

According to Dennett, the same system may be described using a `physical' (mechanical) explanatory stance, or using an `intentional' (belief- and goal-based) explanatory stance. Humans tend to find the physical stance more helpful for certain systems, such as planets orbiting a star, and the intentional stance for others, such as living animals. We define a formal counterpart of physical and intentional stances within computational theory: a description of a system as either a device, or an agent, with the key difference being that `devices' are directly described in terms of an input-output mapping, while `agents' are described in terms of the function they optimise. Bayes' rule can then be applied to calculate the subjective probability of a system being a device or an agent, based only on its behaviour. We illustrate this using the trajectories of an object in a toy grid-world domain.

==> agency-logs/circle-hits.tex <==
empty,down & \_ & \_ & \_ & 6\\
empty,left & \_ & 7 & \_ & \_\\
empty,right & 6 & \_ & \_ & \_\\
empty,up & \_ & \_ & 6 & \_\\


==> agency-logs/circle-posts-v.tex <==
& Device & Agent \\
\hline
$v_1$ & 18.01 & 37.48 \\
$v_2$ & 1.00 & 0.00 \\
$v_3$ & 0.00 & 19.40



==> agency-logs/circle-posts.tex <==
Device & 18.0799 & 1.0000 & 0.0000 \\
Agent & 37.4750 & 0.0000 & 19.3951


==> agency-logs/circle.tex <==
\begin{figure}[htbp!]
\centering
\begin{subfigure}[b]{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{agency-logs/circle.png}
\caption{Trajectory.}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.6\textwidth}
\centering
\begin{tabular}{l | c c c c}
Context & \multicolumn{4}{c}{Action} \\
in\_front,last\_action & up & down & left & right\\
\hline
\input{agency-logs/circle-hits}
\end{tabular}\caption{Contexts hits.}
\end{subfigure}
\\
\begin{subfigure}[b]{\textwidth}
\centering
\caption{Posteriors of the device and agent mixtures.}
\begin{tabular}{l | c c c}
Mixture $\mX$ & $-\ln P(\traj | \mX)$ & $P(\mX | \traj)$ & $-\ln P(\mX | \traj)$ \\
\hline
\input{agency-logs/circle-posts}
\end{tabular}\end{subfigure}
\caption{\captioncircle}%
\label{fig:circle}%
\end{figure}%


==> agency-logs/epsblue-hits.tex <==
darkblue,left & \_ & \_ & 1 & \_\\
empty,down & \_ & 9 & 4 & 3\\
empty,left & 4 & 3 & 6 & \_\\
empty,right & 3 & 3 & \_ & 10\\
empty,up & 4 & \_ & 4 & 1\\
wall,down & \_ & \_ & \_ & 3\\
wall,left & \_ & 2 & \_ & \_\\
wall,right & 1 & 1 & \_ & \_\\
wall,up & 1 & \_ & 2 & 1\\


==> agency-logs/epsblue-posts-v.tex <==
& Device & Agent \\
\hline
$v_1$ & 83.53 & 72.04 \\
$v_2$ & 0.00 & 1.00 \\
$v_3$ & 11.49 & 0.00




==> agency-logs/epsblue-posts.tex <==
Device & 83.5277 & 0.0000 & 11.4858 \\
Agent & 72.0418 & 1.0000 & 0.0000


==> agency-logs/epsblue.tex <==
\begin{figure}[htbp!]
\centering
\begin{subfigure}[b]{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{agency-logs/epsblue.png}
\caption{Trajectory.}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.6\textwidth}
\centering
\begin{tabular}{l | c c c c}
Context & \multicolumn{4}{c}{Action} \\
in\_front,last\_action & up & down & left & right\\
\hline
\input{agency-logs/epsblue-hits}
\end{tabular}\caption{Contexts hits.}
\end{subfigure}
\\
\begin{subfigure}[b]{\textwidth}
\centering
\caption{Posteriors of the device and agent mixtures.}
\begin{tabular}{l | c c c}
Mixture $\mX$ & $-\ln P(\traj | \mX)$ & $P(\mX | \traj)$ & $-\ln P(\mX | \traj)$ \\
\hline
\input{agency-logs/epsblue-posts}
\end{tabular}\end{subfigure}
\caption{\captionepsblue}%
\label{fig:epsblue}%
\end{figure}%


==> agency-logs/followwalls-hits.tex <==
empty,down & \_ & 8 & \_ & \_\\
empty,left & \_ & \_ & 5 & \_\\
empty,right & \_ & \_ & \_ & 8\\
empty,up & 4 & \_ & \_ & \_\\
wall,down & \_ & \_ & \_ & 1\\
wall,left & \_ & 2 & \_ & \_\\
wall,right & 2 & \_ & \_ & \_\\
wall,up & \_ & \_ & 2 & \_\\


==> agency-logs/followwalls-posts-v.tex <==
& Device & Agent \\
\hline
$v_1$ & 26.09 & 43.33 \\
$v_2$ & 1.00 & 0.00 \\
$v_3$ & 0.00 & 17.24




==> agency-logs/followwalls-posts.tex <==
Device & 26.0866 & 1.0000 & 0.0000 \\
Agent & 43.3295 & 0.0000 & 17.2428


==> agency-logs/followwalls.tex <==
\begin{figure}[htbp!]
\centering
\begin{subfigure}[b]{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{agency-logs/followwalls.png}
\caption{Trajectory.}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.6\textwidth}
\centering
\begin{tabular}{l | c c c c}
Context & \multicolumn{4}{c}{Action} \\
in\_front,last\_action & up & down & left & right\\
\hline
\input{agency-logs/followwalls-hits}
\end{tabular}\caption{Contexts hits.}
\end{subfigure}
\\
\begin{subfigure}[b]{\textwidth}
\centering
\caption{Posteriors of the device and agent mixtures.}
\begin{tabular}{l | c c c}
Mixture $\mX$ & $-\ln P(\traj | \mX)$ & $P(\mX | \traj)$ & $-\ln P(\mX | \traj)$ \\
\hline
\input{agency-logs/followwalls-posts}
\end{tabular}\end{subfigure}
\caption{\captionfollowwalls}%
\label{fig:followwalls}%
\end{figure}%


==> agency-logs/magenta-hits.tex <==
empty,down & \_ & 2 & \_ & 1\\
empty,right & \_ & 1 & \_ & 10\\
empty,up & 1 & \_ & \_ & 1\\
magenta,down & \_ & 1 & \_ & \_\\
wall,right & 1 & \_ & \_ & \_\\


==> agency-logs/magenta-posts-v.tex <==
& Device & Agent \\
\hline
$v_1$ & 18.16 & 11.31 \\
$v_2$ & 0.00 & 1.00 \\
$v_3$ & 6.85 & 0.00


==> agency-logs/magenta-posts.tex <==
Device & 18.1577 & 0.0011 & 6.8453 \\
Agent & 11.3135 & 0.9989 & 0.0011


==> agency-logs/magenta.tex <==
\begin{figure}[htbp!]
\centering
\begin{subfigure}[b]{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{agency-logs/magenta.png}
\caption{Trajectory.}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.6\textwidth}
\centering
\begin{tabular}{l | c c c c}
Context & \multicolumn{4}{c}{Action} \\
in\_front,last\_action & up & down & left & right\\
\hline
\input{agency-logs/magenta-hits}
\end{tabular}\caption{Contexts hits.}
\end{subfigure}
\\
\begin{subfigure}[b]{\textwidth}
\centering
\caption{Posteriors of the device and agent mixtures.}
\begin{tabular}{l | c c c}
Mixture $\mX$ & $-\ln P(\traj | \mX)$ & $P(\mX | \traj)$ & $-\ln P(\mX | \traj)$ \\
\hline
\input{agency-logs/magenta-posts}
\end{tabular}\end{subfigure}
\caption{\captionmagenta}%
\label{fig:magenta}%
\end{figure}%


==> agency-logs/random-posts-v.tex <==
& Device & Agent \\
\hline
$v_1$ & 141.64 & 144.11 \\
$v_2$ & 0.92 & 0.08 \\
$v_3$ & 0.08 & 2.55

==> agency-logs/random-posts.tex <==
Device & 141.6367 & 0.9219 & 0.0813 \\
Agent & 144.1054 & 0.0781 & 2.5500


==> agency-logs/random.tex <==
\begin{figure}[htbp!]
\centering
\begin{subfigure}[b]{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{agency-logs/random.png}
\caption{Trajectory.}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.6\textwidth}
\centering
\begin{tabular}{l | c c c c}
Context & \multicolumn{4}{c}{Action} \\
in\_front,last\_action & up & down & left & right\\
\hline
\input{agency-logs/random-hits}
\end{tabular}\caption{Contexts hits.}
\end{subfigure}
\\
\begin{subfigure}[b]{\textwidth}
\centering
\caption{Posteriors of the device and agent mixtures.}
\begin{tabular}{l | c c c}
Mixture $\mX$ & $-\ln P(\traj | \mX)$ & $P(\mX | \traj)$ & $-\ln P(\mX | \traj)$ \\
\hline
\input{agency-logs/random-posts}
\end{tabular}\end{subfigure}
\caption{\captionrandom}%
\label{fig:random}%
\end{figure}%


==> agency-logs/switch.tex <==
\begin{figure}[htbp!]
\centering
\begin{subfigure}[b]{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{agency-logs/switch.png}
\caption{Trajectory.}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.6\textwidth}
\centering
\begin{tabular}{l | c c c c}
Context & \multicolumn{4}{c}{Action} \\
in\_front,last\_action & up & down & left & right\\
\hline
darkblue,left & \_ & \_ & \_ & 1\\
darkgreen,up & 1 & \_ & \_ & \_\\
darkred,down & \_ & \_ & \_ & 1\\
darkred,left & \_ & \_ & 1 & \_\\
empty,down & \_ & 17 & 2 & \_\\
empty,left & 1 & 1 & 20 & \_\\
empty,right & 1 & 1 & \_ & 20\\
empty,up & 6 & 1 & 1 & \_\\
wall,down & \_ & \_ & 1 & 2\\
wall,right & 1 & 2 & \_ & \_\\
wall,up & \_ & \_ & \_ & 1\\
\end{tabular}\caption{Contexts hits.}
\end{subfigure}
\\
\begin{subfigure}[b]{\textwidth}
\centering
\caption{Posteriors of the device and agent mixtures.}
\begin{tabular}{l | c c c}
Mixture $\mX$ & $-\ln P(\traj | \mX)$ & $P(\mX | \traj)$ & $-\ln P(\mX | \traj)$ \\
\hline
Device & 64.4851 & 1.0000 & 0.0000 \\
Agent & 92.1446 & 0.0000 & 27.6595
\end{tabular}\end{subfigure}
\caption{\captionswitch}%
\label{fig:switch}%
\end{figure}%


==> agency-logs/switchB-hits.tex <==
darkblue,left & \_ & \_ & \_ & 1\\
darkgreen,up & 1 & \_ & \_ & \_\\
darkred,down & \_ & \_ & \_ & 1\\
darkred,left & \_ & \_ & 1 & \_\\
empty,down & \_ & 17 & 2 & \_\\
empty,left & 1 & 1 & 20 & \_\\
empty,right & 1 & 1 & \_ & 20\\
empty,up & 6 & 1 & 1 & \_\\
wall,down & \_ & \_ & 1 & 2\\
wall,right & 1 & 2 & \_ & \_\\
wall,up & \_ & \_ & \_ & 1\\


==> agency-logs/switchB-posts.tex <==
Device & 64.4851 & 0.0000 & 34.1808 \\
Agent (switching prior) & 30.3043 & 1.0000 & 0.0000 \\
Agent (no switching) & 92.1446 & NA & NA


==> agency-logs/switchB.tex <==
\begin{figure}[htbp!]
\centering
\begin{subfigure}[b]{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{agency-logs/switchB.png}
\caption{Trajectory.}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.6\textwidth}
\centering
\begin{tabular}{l | c c c c}
Context & \multicolumn{4}{c}{Action} \\
in\_front,last\_action & up & down & left & right\\
\hline
\input{agency-logs/switchB-hits}
\end{tabular}\caption{Contexts hits.}
\end{subfigure}
\\
\begin{subfigure}[b]{\textwidth}
\centering
\caption{Posteriors of the device and agent mixtures.}
\begin{tabular}{l | c c c}
Mixture $\mX$ & $-\ln P(\traj | \mX)$ & $P(\mX | \traj)$ & $-\ln P(\mX | \traj)$ \\
\hline
\input{agency-logs/switchB-posts}
\end{tabular}\end{subfigure}
\caption{\captionswitchB}%
\label{fig:switchB}%
\end{figure}%


==> notation.tex <==


